Train Till You Drop: Towards Stable and Robust Source-free Unsupervised 3D Domain Adaptation

We tackle the challenging problem of source-free unsupervised domain adaptation (SFUDA) for 3D semantic segmentation. It amounts to performing domain adaptation on an unlabeled target domain without any access to source data; the available information is a model trained to achieve good performance on the source domain. A common issue with existing SFUDA approaches is that performance degrades after some training time, which is a by product of an under-constrained and ill-posed problem. We discuss two strategies to alleviate this issue. First, we propose a sensible way to regularize the learning problem. Second, we introduce a novel criterion based on agreement with a reference model. It is used (1) to stop the training when appropriate and (2) as validator to select hyperparameters without any knowledge on the target domain. Our contributions are easy to implement and readily amenable for all SFUDA methods, ensuring stable improvements over all baselines. We validate our findings on various 3D lidar settings, achieving state-of-the-art performance. The project repository (with code) is: github.com/valeoai/TTYD.

==> figures/main_figure_data/ns2sk/ttyd_training.tex <==
0 34.40932035446167
1 38.94598186016083
2 42.4412190914154
3 43.87383460998535
4 44.44973766803741
5 44.6181982755661
6 44.54650282859802
7 44.51648890972137
8 44.3576455116272
9 44.043275713920586
10 43.76656413078308
11 43.35483014583587
12 43.15338134765625
13 42.95455813407898
14 42.61317253112793
15 42.37464368343353
16 42.09001958370209
17 41.8202131986618
18 41.53857827186584
19 41.37549102306366
20 41.22543036937713

==> figures/rebuttal_eccv/ablation_lr/ns2pd/criterion/lr_10_1.tex <==
0	91.71
1	15.90
2	10.71

==> figures/rebuttal_eccv/ablation_lr/ns2pd/criterion/lr_10_2.tex <==
0	91.71
1	78.12
2	75.80
3	75.51
4	73.00
5	73.82
6	69.46
7	66.55
8	71.20
9	72.01
10	68.80
11	67.78
12	69.25
13	69.28
14	61.97
15	62.38
16	54.30
17	59.09
18	54.04
19	46.33

==> figures/rebuttal_eccv/ablation_lr/ns2pd/criterion/lr_10_3.tex <==
0	91.75
1	81.41
2	83.87
3	80.19
4	87.42
5	78.03
6	77.35
7	82.60
8	82.23
9	83.65
10	82.22
11	81.66
12	78.27
13	77.99
14	77.49
15	77.10
16	75.77
17	80.31
18	81.63
19	81.36

==> figures/rebuttal_eccv/ablation_lr/ns2pd/criterion/lr_10_4.tex <==
0	91.75
1	87.50
2	86.87
3	85.32
4	84.22
5	83.12
6	80.74
7	79.88
8	80.74
9	80.95
10	82.80
11	83.14
12	82.23
13	80.99
14	80.94
15	81.37
16	81.84
17	81.89
18	81.87
19	80.94

==> figures/rebuttal_eccv/ablation_lr/ns2pd/criterion/lr_10_5.tex <==
0	91.74
1	93.34
2	92.58
3	91.44
4	90.65
5	89.94
6	89.50
7	89.04
8	88.57
9	88.22
10	87.97
11	87.77
12	87.28
13	87.13
14	86.97
15	87.03
16	86.99
17	86.89
18	86.71
19	86.47

==> figures/rebuttal_eccv/ablation_lr/ns2pd/criterion/lr_10_6.tex <==
0	91.73
1	92.15
2	92.42
3	92.75
4	92.94
5	93.07
6	93.21
7	93.26
8	93.26
9	93.30
10	93.26
11	93.25
12	93.22
13	93.15
14	93.07
15	92.92
16	92.86
17	92.73
18	92.56
19	92.45

==> figures/rebuttal_eccv/ablation_lr/ns2pd/criterion/lr_10_7.tex <==
0	91.70
1	91.79
2	91.80
3	91.85
4	91.93
5	91.90
6	92.02
7	92.04
8	92.06
9	92.09
10	92.16
11	92.13
12	92.24
13	92.28
14	92.30
15	92.30
16	92.38
17	92.38
18	92.41
19	92.44

==> figures/rebuttal_eccv/ablation_lr/ns2pd/miou/lr_10_1.tex <==
0	60.38
1	6.95
2	5.59

==> figures/rebuttal_eccv/ablation_lr/ns2pd/miou/lr_10_2.tex <==
0	60.38
1	43.55
2	40.95
3	39.13
4	36.39
5	34.79
6	32.67
7	29.15
8	31.20
9	32.56
10	29.92
11	29.38
12	30.23
13	29.02
14	26.08
15	25.58
16	23.21
17	24.56
18	22.26
19	16.04

==> figures/rebuttal_eccv/ablation_lr/ns2pd/miou/lr_10_3.tex <==
0	60.38
1	53.61
2	56.04
3	52.93
4	59.60
5	51.16
6	50.16
7	55.89
8	55.32
9	53.95
10	53.55
11	52.72
12	45.75
13	45.12
14	44.43
15	43.66
16	42.72
17	48.88
18	50.42
19	49.99

==> figures/rebuttal_eccv/ablation_lr/ns2pd/miou/lr_10_4.tex <==
0	60.38
1	62.54
2	61.59
3	59.74
4	58.52
5	57.19
6	54.24
7	53.02
8	53.93
9	54.19
10	56.45
11	56.99
12	56.03
13	54.16
14	54.10
15	54.32
16	54.74
17	54.69
18	54.37
19	53.41

==> figures/rebuttal_eccv/ablation_lr/ns2pd/miou/lr_10_5.tex <==
0	60.38
1	63.35
2	64.49
3	64.86
4	64.70
5	64.38
6	64.01
7	63.57
8	63.12
9	62.75
10	62.42
11	62.12
12	61.62
13	61.35
14	61.19
15	61.15
16	61.03
17	60.84
18	60.58
19	60.35

==> figures/rebuttal_eccv/ablation_lr/ns2pd/miou/lr_10_6.tex <==
0	60.38
1	60.86
2	61.27
3	61.65
4	61.98
5	62.29
6	62.57
7	62.83
8	63.06
9	63.27
10	63.46
11	63.63
12	63.80
13	63.96
14	64.09
15	64.21
16	64.32
17	64.41
18	64.50
19	64.58

==> figures/rebuttal_eccv/ablation_lr/ns2pd/miou/lr_10_7.tex <==
0	60.38
1	60.43
2	60.48
3	60.53
4	60.58
5	60.63
6	60.68
7	60.73
8	60.78
9	60.82
10	60.87
11	60.92
12	60.96
13	61.01
14	61.05
15	61.10
16	61.14
17	61.18
18	61.23
19	61.27

==> figures/rebuttal_eccv/ablation_lr/ns2poss/criterion/lr_10_2.tex <==
0	87.94
1	46.98
2	45.93
3	41.11
4	35.31
5	37.67
6	45.10
7	43.95
8	43.75
9	41.54
10	45.84
11	20.43
12	23.82
13	20.67
14	18.42
15	7.48
16	8.75
17	19.13
18	17.32
19	27.52

==> figures/rebuttal_eccv/ablation_lr/ns2poss/criterion/lr_10_3.tex <==
0	87.93
1	47.09
2	46.53
3	46.16
4	40.03
5	40.84
6	40.81
7	40.74
8	40.69
9	40.62
10	40.60
11	40.59
12	40.56
13	40.11
14	40.11
15	40.09
16	40.02
17	39.99
18	40.26
19	40.41

==> figures/rebuttal_eccv/ablation_lr/ns2poss/criterion/lr_10_4.tex <==
0	87.93
1	52.92
2	46.48
3	45.94
4	44.97
5	44.84
6	43.98
7	44.19
8	44.14
9	44.07
10	43.29
11	43.31
12	43.23
13	42.60
14	42.55
15	42.53
16	42.50
17	42.44
18	42.36
19	42.39

==> figures/rebuttal_eccv/ablation_lr/ns2poss/criterion/lr_10_5.tex <==
0	87.97
1	92.23
2	92.16
3	91.03
4	86.35
5	80.68
6	75.41
7	67.13
8	61.91
9	56.89
10	52.12
11	49.93
12	48.81
13	48.11
14	47.69
15	47.39
16	47.12
17	46.77
18	46.64
19	46.52

==> figures/rebuttal_eccv/ablation_lr/ns2poss/criterion/lr_10_6.tex <==
0	87.91
1	88.75
2	89.45
3	90.14
4	90.71
5	91.17
6	91.53
7	91.83
8	92.01
9	92.07
10	92.13
11	92.14
12	92.18
13	92.18
14	92.21
15	92.26
16	92.23
17	92.21
18	92.19
19	92.18

==> figures/rebuttal_eccv/ablation_lr/ns2poss/criterion/lr_10_7.tex <==
0	87.82
1	87.91
2	88.12
3	88.11
4	88.27
5	88.39
6	88.41
7	88.59
8	88.60
9	88.71
10	88.83
11	88.86
12	88.93
13	89.02
14	89.16
15	89.20
16	89.23
17	89.31
18	89.43
19	89.54

==> figures/rebuttal_eccv/ablation_lr/ns2poss/miou/lr_10_2.tex <==
0	60.42
1	25.28
2	21.50
3	16.75
4	13.88
5	13.82
6	16.00
7	15.20
8	15.38
9	14.72
10	14.42
11	11.26
12	13.74
13	12.73
14	11.65
15	14.21
16	15.21
17	14.53
18	13.25
19	12.03

==> figures/rebuttal_eccv/ablation_lr/ns2poss/miou/lr_10_3.tex <==
0	60.42
1	25.23
2	24.77
3	24.37
4	18.15
5	19.17
6	19.14
7	19.11
8	19.26
9	19.26
10	19.25
11	19.24
12	19.23
13	18.99
14	18.95
15	18.91
16	18.86
17	18.81
18	19.23
19	19.40

==> figures/rebuttal_eccv/ablation_lr/ns2poss/miou/lr_10_4.tex <==
0	60.42
1	31.21
2	24.69
3	24.07
4	23.09
5	22.73
6	21.80
7	22.10
8	22.06
9	22.02
10	21.16
11	21.12
12	21.08
13	20.49
14	20.46
15	20.43
16	20.39
17	20.36
18	20.33
19	20.30

==> figures/rebuttal_eccv/ablation_lr/ns2poss/miou/lr_10_5.tex <==
0	60.42
1	61.43
2	60.99
3	60.06
4	57.43
5	54.18
6	51.16
7	45.36
8	40.46
9	35.15
10	30.27
11	28.13
12	26.98
13	26.33
14	25.84
15	25.47
16	25.17
17	24.86
18	24.66
19	24.56

==> figures/rebuttal_eccv/ablation_lr/ns2poss/miou/lr_10_6.tex <==
0	60.42
1	60.67
2	60.87
3	61.04
4	61.18
5	61.28
6	61.36
7	61.41
8	61.43
9	61.45
10	61.44
11	61.42
12	61.39
13	61.36
14	61.33
15	61.29
16	61.25
17	61.22
18	61.18
19	61.13

==> figures/rebuttal_eccv/ablation_lr/ns2poss/miou/lr_10_7.tex <==
0	60.42
1	60.45
2	60.48
3	60.51
4	60.53
5	60.56
6	60.58
7	60.61
8	60.63
9	60.66
10	60.68
11	60.70
12	60.73
13	60.75
14	60.77
15	60.79
16	60.81
17	60.83
18	60.85
19	60.87

==> figures/rebuttal_eccv/ablation_lr/ns2wy/criterion/lr_10_1.tex <==
0	84.42
1	7.24
2	3.52
3	5.92
4	5.94
5	4.72
6	9.52
7	8.31
8	7.93

==> figures/rebuttal_eccv/ablation_lr/ns2wy/criterion/lr_10_2.tex <==
0	84.41
1	76.49
2	62.45
3	53.54
4	49.25
5	47.04
6	52.00
7	46.66
8	37.89
9	46.37
10	48.84
11	29.70
12	38.20

==> figures/rebuttal_eccv/ablation_lr/ns2wy/criterion/lr_10_3.tex <==
0	84.43
1	84.16
2	81.76
3	79.81
4	75.36
5	79.48
6	81.51
7	76.23
8	75.48
9	69.82
10	68.98
11	76.78
12	69.16

==> figures/rebuttal_eccv/ablation_lr/ns2wy/criterion/lr_10_4.tex <==
0	84.42
1	88.37
2	86.97
3	86.23
4	85.45
5	85.46
6	85.28
7	84.58
8	83.76
9	83.10
10	82.93
11	82.93
12	82.66

==> figures/rebuttal_eccv/ablation_lr/ns2wy/criterion/lr_10_5.tex <==
0	84.40
1	88.32
2	89.59
3	89.87
4	89.71
5	89.35
6	88.93
7	88.51
8	88.12
9	87.78
10	87.47
11	87.17
12	87.03

==> figures/rebuttal_eccv/ablation_lr/ns2wy/criterion/lr_10_6.tex <==
0	84.42
1	85.06
2	85.57
3	86.05
4	86.49
5	86.91
6	87.30
7	87.61
8	87.90
9	88.19
10	88.39
11	88.64
12	88.84

==> figures/rebuttal_eccv/ablation_lr/ns2wy/criterion/lr_10_7.tex <==
0	84.42
1	84.48
2	84.55
3	84.59
4	84.69
5	84.72
6	84.80
7	84.86
8	84.93
9	85.01
10	85.03
11	85.10
12	85.17

==> figures/rebuttal_eccv/ablation_lr/ns2wy/miou/lr_10_1.tex <==
0	46.08
1	3.89
2	3.07
3	2.99
4	3.01
5	2.32
6	2.86
7	3.73
8	3.37

==> figures/rebuttal_eccv/ablation_lr/ns2wy/miou/lr_10_2.tex <==
0	46.08
1	33.26
2	21.58
3	19.39
4	17.45
5	15.21
6	15.21
7	15.09
8	10.85
9	11.12
10	12.20
11	8.95
12	10.49

==> figures/rebuttal_eccv/ablation_lr/ns2wy/miou/lr_10_3.tex <==
0	46.08
1	43.71
2	40.58
3	37.23
4	34.73
5	36.29
6	38.20
7	33.33
8	32.00
9	29.35
10	28.54
11	33.29
12	30.04

==> figures/rebuttal_eccv/ablation_lr/ns2wy/miou/lr_10_4.tex <==
0	46.08
1	50.40
2	48.68
3	47.63
4	46.49
5	46.05
6	45.79
7	44.90
8	43.65
9	42.81
10	42.47
11	42.41
12	41.84

==> figures/rebuttal_eccv/ablation_lr/ns2wy/miou/lr_10_5.tex <==
0	46.08
1	49.81
2	51.07
3	51.38
4	51.35
5	51.13
6	50.79
7	50.48
8	50.10
9	49.76
10	49.41
11	49.08
12	48.90

==> figures/rebuttal_eccv/ablation_lr/ns2wy/miou/lr_10_6.tex <==
0	46.08
1	46.66
2	47.17
3	47.66
4	48.09
5	48.47
6	48.83
7	49.14
8	49.41
9	49.67
10	49.90
11	50.11
12	50.29

==> figures/rebuttal_eccv/ablation_lr/ns2wy/miou/lr_10_7.tex <==
0	46.08
1	46.14
2	46.20
3	46.26
4	46.32
5	46.38
6	46.44
7	46.50
8	46.55
9	46.61
10	46.67
11	46.73
12	46.79

==> figures/rebuttal_eccv/ablation_lr/syn2poss/criterion/lr_10_1.tex <==
0	10.71
1	11.58
2	11.60
3	11.59
4	11.64
5	11.59
6	11.57
7	11.60
8	11.61
9	11.54
10	11.61
11	11.56
12	11.62
13	11.62
14	11.55
15	11.56
16	11.66
17	11.58
18	11.57
19	11.60

==> figures/rebuttal_eccv/ablation_lr/syn2poss/criterion/lr_10_2.tex <==
0	57.17
1	43.61
2	36.50
3	40.06
4	35.76
5	36.59
6	15.53
7	16.46
8	15.17
9	11.40
10	9.72
11	9.14
12	13.39
13	12.11
14	4.47
15	7.25
16	4.93
17	11.59
18	9.25
19	5.97

==> figures/rebuttal_eccv/ablation_lr/syn2poss/criterion/lr_10_3.tex <==
0	57.14
1	49.41
2	49.11
3	48.32
4	38.07
5	37.34
6	33.35
7	32.79
8	32.28
9	31.80
10	31.75
11	31.20
12	30.61
13	30.01
14	29.42
15	28.82
16	28.18
17	27.64
18	27.08
19	26.48

==> figures/rebuttal_eccv/ablation_lr/syn2poss/criterion/lr_10_4.tex <==
0	57.23
1	57.83
2	52.96
3	52.60
4	51.25
5	51.32
6	50.37
7	47.43
8	48.92
9	48.82
10	50.78
11	50.96
12	48.72
13	48.74
14	48.56
15	48.59
16	48.48
17	48.34
18	45.29
19	45.21

==> figures/rebuttal_eccv/ablation_lr/syn2poss/criterion/lr_10_5.tex <==
0	57.25
1	61.92
2	63.49
3	63.67
4	63.07
5	61.86
6	60.68
7	59.36
8	57.75
9	56.41
10	55.19
11	54.40
12	54.02
13	53.84
14	53.82
15	53.49
16	53.35
17	53.29
18	53.00
19	52.92

==> figures/rebuttal_eccv/ablation_lr/syn2poss/criterion/lr_10_6.tex <==
0	56.23
1	56.96
2	57.55
3	58.17
4	58.79
5	59.25
6	59.76
7	60.19
8	60.70
9	60.91
10	61.28
11	61.60
12	61.79
13	62.10
14	62.26
15	62.43
16	62.78
17	63.03
18	63.29
19	63.53

==> figures/rebuttal_eccv/ablation_lr/syn2poss/criterion/lr_10_7.tex <==
0	57.23
1	57.33
2	57.38
3	57.44
4	57.54
5	57.61
6	57.62
7	57.84
8	57.75
9	57.86
10	57.99
11	58.04
12	58.02
13	58.23
14	58.27
15	58.34
16	58.40
17	58.50
18	58.51
19	58.53

==> figures/rebuttal_eccv/ablation_lr/syn2poss/miou/lr_10_1.tex <==
0	25.59
1	5.41
2	5.41
3	5.41
4	5.41
5	5.41
6	5.41
7	5.41
8	5.41
9	5.41
10	5.41
11	5.41
12	5.41
13	5.41
14	5.41
15	5.41
16	5.41
17	5.41
18	5.41
19	5.41

==> figures/rebuttal_eccv/ablation_lr/syn2poss/miou/lr_10_2.tex <==
0	25.59
1	17.78
2	13.95
3	12.52
4	8.62
5	8.58
6	7.89
7	8.07
8	7.07
9	7.24
10	7.21
11	5.53
12	5.42
13	5.61
14	5.81
15	4.43
16	3.11
17	4.18
18	4.12
19	4.46

==> figures/rebuttal_eccv/ablation_lr/syn2poss/miou/lr_10_3.tex <==
0	25.59
1	27.49
2	26.39
3	25.93
4	21.35
5	20.96
6	16.94
7	16.42
8	15.85
9	15.29
10	15.89
11	15.37
12	14.86
13	14.35
14	13.81
15	13.25
16	12.68
17	12.13
18	11.59

==> figures/rebuttal_eccv/ablation_lr/syn2poss/miou/lr_10_4.tex <==
0	25.59
1	32.37
2	29.90
3	29.62
4	28.93
5	28.89
6	28.42
7	26.91
8	27.62
9	27.57
10	28.50
11	28.56
12	27.45
13	27.42
14	27.38
15	27.34
16	27.30
17	27.26
18	25.49

==> figures/rebuttal_eccv/ablation_lr/syn2poss/miou/lr_10_5.tex <==
0	25.59
1	32.26
2	34.93
3	35.91
4	35.96
5	35.53
6	34.76
7	33.77
8	32.80
9	32.16
10	31.60
11	31.13
12	30.93
13	30.80
14	30.74
15	30.58
16	30.49
17	30.43
18	30.32
19	30.20

==> figures/rebuttal_eccv/ablation_lr/syn2poss/miou/lr_10_6.tex <==
0	25.59
1	26.49
2	27.35
3	28.19
4	28.99
5	29.72
6	30.42
7	31.06
8	31.67
9	32.21
10	32.71
11	33.16
12	33.56
13	33.92
14	34.24
15	34.52
16	34.78
17	34.99
18	35.18
19	35.35

==> figures/rebuttal_eccv/ablation_lr/syn2poss/miou/lr_10_7.tex <==
0	25.59
1	25.69
2	25.78
3	25.88
4	25.97
5	26.07
6	26.16
7	26.26
8	26.35
9	26.45
10	26.54
11	26.64
12	26.74
13	26.83
14	26.93
15	27.02
16	27.11
17	27.21
18	27.30
19	27.40

==> figures/rebuttal_eccv/ablation_lr/syn2sk/criterion/lr_10_1.tex <==
0	58.46
1	58.43
2	58.42
3	58.37
4	58.35
5	58.40
6	58.41
7	58.39
8	58.34
9	58.42
10	58.37
11	58.35
12	58.42
13	58.44
14	58.45
15	58.41
16	58.42
17	58.36
18	58.43
19	58.39

==> figures/rebuttal_eccv/ablation_lr/syn2sk/criterion/lr_10_2.tex <==
0	58.43
1	48.99
2	47.78
3	35.92
4	36.65
5	31.28
6	22.32
7	30.70
8	32.91
9	29.25
10	30.43
11	30.19
12	32.12
13	30.31
14	27.43
15	28.46
16	26.70
17	27.99
18	26.81
19	26.41

==> figures/rebuttal_eccv/ablation_lr/syn2sk/criterion/lr_10_3.tex <==
0	58.35
1	69.07
2	62.77
3	65.52
4	63.36
5	62.53
6	58.84
7	58.01
8	57.38
9	56.61
10	52.69
11	52.92
12	58.03
13	51.74
14	49.98
15	52.48
16	52.30
17	52.09
18	48.29
19	50.88

==> figures/rebuttal_eccv/ablation_lr/syn2sk/criterion/lr_10_4.tex <==
0	58.39
1	73.63
2	72.23
3	71.77
4	71.89
5	71.45
6	70.53
7	70.85
8	69.98
9	69.32
10	67.14
11	67.96
12	67.32
13	66.77
14	66.36
15	67.65
16	67.45
17	65.88
18	68.44
19	67.86

==> figures/rebuttal_eccv/ablation_lr/syn2sk/criterion/lr_10_5.tex <==
0	58.38
1	65.89
2	70.47
3	72.53
4	73.44
5	73.74
6	73.87
7	73.75
8	73.60
9	73.47
10	73.40
11	73.30
12	73.29
13	73.12
14	73.05
15	73.01
16	72.96
17	72.93
18	72.72
19	72.54

==> figures/rebuttal_eccv/ablation_lr/syn2sk/criterion/lr_10_6.tex <==
0	58.40
1	59.31
2	60.14
3	61.01
4	61.81
5	62.57
6	63.32
7	64.11
8	64.75
9	65.48
10	66.00
11	66.72
12	67.29
13	67.81
14	68.39
15	68.87
16	69.29
17	69.72
18	70.04
19	70.44

==> figures/rebuttal_eccv/ablation_lr/syn2sk/criterion/lr_10_7.tex <==
0	58.51486325
1	58.53037834
2	58.58361125
3	58.64180326
4	58.75593424
5	58.82116556
6	58.94711018
7	59.0200603
8	59.1321826
9	59.25349593
10	59.25211906

==> figures/rebuttal_eccv/ablation_lr/syn2sk/miou/lr_10_1.tex <==
0	22.29
1	22.29
2	22.29
3	22.29
4	22.29
5	22.29
6	22.29
7	22.29
8	22.29
9	22.29
10	22.29
11	22.29
12	22.29
13	22.29
14	22.29
15	22.29
16	22.29
17	22.29
18	22.29
19	0.00

==> figures/rebuttal_eccv/ablation_lr/syn2sk/miou/lr_10_2.tex <==
0	22.29
1	16.81
2	12.31
3	7.84
4	7.99
5	4.28
6	3.37
7	5.02
8	4.93
9	4.71
10	4.66
11	4.21
12	4.16
13	4.91
14	4.93
15	4.99
16	4.42
17	4.63
18	3.90
19	3.87

==> figures/rebuttal_eccv/ablation_lr/syn2sk/miou/lr_10_3.tex <==
0	22.29
1	24.64
2	22.25
3	21.47
4	20.51
5	20.15
6	18.90
7	17.92
8	17.63
9	17.34
10	17.18
11	16.56
12	19.49
13	14.83
14	13.47
15	15.84
16	15.72
17	15.61
18	13.74
19	13.07

==> figures/rebuttal_eccv/ablation_lr/syn2sk/miou/lr_10_4.tex <==
0	22.29
1	28.41
2	27.96
3	27.46
4	27.41
5	27.06
6	26.44
7	25.95
8	25.45
9	25.75
10	24.46
11	24.84
12	24.57
13	24.36
14	23.88
15	24.08
16	24.05
17	23.12
18	24.20
19	23.81

==> figures/rebuttal_eccv/ablation_lr/syn2sk/miou/lr_10_5.tex <==
0	22.29
1	24.64
2	26.13
3	26.99
4	27.51
5	27.82
6	28.06
7	28.17
8	28.25
9	28.27
10	28.25
11	28.22
12	28.17
13	28.08
14	28.03
15	28.04
16	27.92
17	27.88
18	27.84
19	27.67

==> figures/rebuttal_eccv/ablation_lr/syn2sk/miou/lr_10_6.tex <==
0	22.29
1	22.59
2	22.86
3	23.12
4	23.37
5	23.60
6	23.83
7	24.05
8	24.27
9	24.48
10	24.67
11	24.88
12	25.05
13	25.23
14	25.40
15	25.55
16	25.69
17	25.82
18	25.95
19	26.07

==> figures/rebuttal_eccv/ablation_lr/syn2sk/miou/lr_10_7.tex <==
0	22.29431421
1	22.32210189
2	22.35134691
3	22.38069326
4	22.40933776
5	22.43856639
6	22.46665955
7	22.49662876
8	22.52634615
9	22.55551517
10	22.58533388

==> tables/class_mappings/ns2pd.tex <==
\begin{table}[!t]
    \small
    \setlength{\tabcolsep}{2pt}
    \centering
    \caption{Class mapping for \nstopd\ (from~\cite{Sanchez_2023_ICCV}).}
\label{tab:app:class_mapping_ns_pd}
        \begin{tabular}{c|c|c}
            \toprule
\rowcolor{violet!10}           
             nuScenes & \nstopd & Pandaset \\ 
             \bottomrule \vphantom{$X^{X^X}$}
              & \multirow{ 4}{*}{2-wheeled} & Bicycle, Motorcycle,   \\
           Bicycle,  && Motorized scooter\\
           Motorcycle && Pedicab, \\
            && Personal Mobility Device\\
            
            \midrule
            \multirow{ 2}{*}{Pedestrian} & \multirow{2}{*}{Pedestrian} & Pedestrian,\\ & &Pedestrian w/ objects \\
            \midrule
            \multirow{ 2}{*}{Driveable ground} & \multirow{ 2}{*}{Driveable ground} & Driveway, Road,\\
            && Road marking \\
            \midrule
            Sidewalk & Sidewalk & Sidewalk\\
            \midrule
            Other flat, Terrain& Other ground & Ground \\
            \midrule
              & \multirow{ 5}{*}{Manmade} &Building, Cones,      \\
            Barrier, && Construction Barriers/Signs, \\
             Manmade,&&  Other static object,\\
            Traffic cone&& Pylons, Road Barriers, \\
            && Rolling containers, Signs \\
                

            
            \midrule
            Vegetation & Vegetation & Vegetation\\
            \midrule
               &\multirow{ 5}{*}{4-wheeled} & Car, Construction vehicle,   \\
             Bus, Car,&& Emergency vehicle,\\ 
             Construction vehicle,&&Bus, Towed object, \\
            Trailer, Truck && Truck (all kinds of)\\   \\
            && Uncommon vehicle\\

            
           
            \bottomrule
        \end{tabular}
      
\end{table}

==> tables/class_mappings/ns2poss.tex <==
\begin{table}[!p]
    \small
    \setlength{\tabcolsep}{2pt}
    \centering

    \caption{Class mapping for \nstoposs\ (from~\cite{Sanchez_2023_ICCV}).}
\label{tab:app:class_mapping_ns_poss}
        \begin{tabular}{c|c|c}
            \toprule
            
\rowcolor{violet!10}                      
            nuScenes & \nstoposs & SemanticPOSS \\ 
             \bottomrule \vphantom{$X^{X^X}$}
            Pedestrian & Person & Person \\
            \midrule
            Bicycle, Motorcycle& Bike & Rider, Bike \\
            \midrule
            Car, Bus, & \multirow{ 3}{*}{Car} & \multirow{ 3}{*}{Car} \\
            Constriction vehicle,&&\\
            Trailer,Truck&&\\
            \midrule
            Driveable surface, Other flat, & \multirow{ 2}{*}{Ground} & \multirow{ 2}{*}{Ground} \\
             Sidewalk, Terrain&&\\
             \midrule
            Vegetation & Vegetation &  Plants \\
            \midrule
            Barrier,  & \multirow{ 3}{*}{Manmade} & Traffic sign, Pole,  \\
            Manmade,  &&  Garbage can, Building, \\
            Traffic cone & &  Cone/Stone, Fence\\
            

            \bottomrule
        \end{tabular}
       
\end{table}

==> tables/class_mappings/ns2sk.tex <==
\begin{table}[!p]
    \small
    \setlength{\tabcolsep}{2pt}
    \centering
    \caption{Class mapping for \nstosk\ (from~\cite{yi2021complete}).}
\label{tab:app:class_mapping_ns_sk}
        \begin{tabular}{c|c|c}
            \toprule
              
\rowcolor{violet!10}           
            nuScenes & \nstosk & SemanticKITTI \\ 
             %\midrule
             \bottomrule \vphantom{$X^{X^X}$}
            Car & Car &  Car\\
            \midrule
            Bicycle    & Bicycle & Bicycle \\
            \midrule
            Motorcycle & Motorcycle & Motorcycle \\
            \midrule
            Truck   & Truck & Truck \\
            \midrule
            Construction  &  \multirow{ 2}{*}{Other vehicle} &  Other-vehicle, \\
            vehicle, Bus & & Bus \\
            \midrule
            Pedestrian  & Pedestrian & Person \\
            \midrule
            \multirow{ 3}{*}{\shortstack{Driveable \\ Surface}}    & \multirow{ 3}{*}{\shortstack{Driveable \\ surface}} & Road,\\
            & & Parking,\\
            & & Lane marking \\
            \midrule
            Sidewalk   & Sidewalk &  Sidewalk \\
            \midrule
            Terrain    & Terrain &  Terrain\\
            \midrule
            Vegetation  & Vegetation & Vegetation, Trunk\\ 
            

            \bottomrule
        \end{tabular}

\end{table}




==> tables/class_mappings/ns2wy.tex <==
\begin{table}[!p]
    \small
    \setlength{\tabcolsep}{2pt}
    \centering

    \caption{Class mapping for \nstowy\ (from~\cite{kim2023single}).}
\label{tab:app:class_mapping_ns_wy}
        \begin{tabular}{c|c|c}
            \toprule
              
\rowcolor{violet!10}                      
            nuScenes & \nstowy & Waymo Open \\ 
             \bottomrule \vphantom{$X^{X^X}$}
            Pedestrian & Person & Person \\
            \midrule
            Bicycle, Motorcycle& Bike & Rider, Bike \\
            \midrule
            Car, Bus, & \multirow{ 3}{*}{Car} & \multirow{ 3}{*}{Car} \\
            Constriction Vehicle,&&\\
            Trailer,Truck&&\\
            \midrule
            Driveable Surface, Other Flat, & \multirow{ 2}{*}{Ground} & \multirow{ 2}{*}{Ground} \\
             Sidewalk, Terrain&&\\
             \midrule
            Vegetation & Vegetation & Vegetation, Plant \\
            \midrule
            Barrier,  & \multirow{ 3}{*}{Manmade} & Traffic Sign, Pole,  \\
            Manmade,  &&  Garbage Can, Building, \\
            Traffic Cone & &  Cone/Stone, Fence\\
            

            \bottomrule
        \end{tabular}
      
\end{table}

==> tables/class_mappings/syn2poss.tex <==
\begin{table}[p!]
    \small
    \setlength{\tabcolsep}{2pt}
    \centering
    \caption{Class mapping for \synthtoposs\ (from~\cite{saltori2022cosmix}).}
\label{tab:app:class_mapping_syn_poss}
        \begin{tabular}{c|c}
            \toprule
              
\rowcolor{violet!10}           
           
            SynLidar & \synthtoposs{} \&  SemanticPOSS \\ 
             \bottomrule \vphantom{$X^{X^X}$}
          Person  & Person  \\
          \midrule
          Bicyclist,Motorcyclist  & Rider  \\
          \midrule
           Car & Car  \\
           \midrule
           Trunk & Trunk  \\
           \midrule
           Vegetation & Plants \\
           \midrule
          Traffic sign  & Traffic sign  \\
          \midrule
          Pole  & Pole \\
          \midrule
          Garbage can  & Garbage can  \\
          \midrule
          Building  & Building  \\
          \midrule
          Traffic-cone  & Cone  \\
          \midrule
          Fence  & Fence \\
          \midrule
          Bicycle  & Bike  \\
          \midrule
          Road  & Ground  \\
            

            \bottomrule
        \end{tabular}
        
\end{table}

==> tables/class_mappings/syn2sk.tex <==
\begin{table}[p!]
    \small
    \setlength{\tabcolsep}{2pt}
    \centering
    \caption{Class mapping for \synthtosk\ (from~\cite{saltori2022cosmix}).}
\label{tab:app:class_mapping_syn_sk}
        \begin{tabular}{c|c}
            \toprule
              
\rowcolor{violet!10}           
           
            SynLiDAR & \synthtosk{} \&  SemanticKITTI \\ 
             \bottomrule \vphantom{$X^{X^X}$}
           Car &Car \\
           \midrule
           Bicycle & Bicycle \\
           \midrule
           Motorcycle & Motorcycle  \\
           \midrule
           Truck & Truck  \\
           \midrule
           Bus, Other vehicle & Other vehicle  \\
           \midrule
           Person & Pedestrian  \\
           \midrule
           Bicyclist & Bicyclist  \\
            \midrule
           Motorcyclist & Motorcyclist  \\
            \midrule
          Road  & Road  \\
           \midrule
          Parking  & Parking  \\
           \midrule
           Sidewalk & Sidewalk  \\
            \midrule
           Other ground & Other ground  \\
            \midrule
          Building  & Building  \\
           \midrule
          Fence  & Fence  \\
           \midrule
          Vegetation  & Vegetation  \\
          \midrule
          Trunk  & Trunk  \\
          \midrule
          Terrain  & Terrain  \\
          \midrule
          Pole  & Pole  \\
          \midrule
          Traffic sign  & Traffic sign \\
            

            \bottomrule
        \end{tabular}
       
\end{table}
